Mining Diamonds in labeled Transition Systems

Labeled transition systems can be a great way to visualize the complex behavior of parallel and communicating systems. However, if, during a particular timeframe, no synchronization or communication between processes occurs, then multiple parallel sequences of actions are able to interleave arbitrarily, and the resulting graph quickly becomes too complex for the human eye to understand easily. With that in mind, we propose an exact formalization of these arbitrary interleavings, and an algorithm to find all said interleavings in deterministic LTSs, to reduce the visual complexity of labeled transition systems.

==> algorithms/exclusive-diamond-singleq.tex <==

\begin{algorithm}[h]
\label{alg:exclusive-diamond-singleq}
\caption{This algorithm finds the possible (exclusive) diamond in a given state, given that only said diamond is available in the given state.}\label{alg:two}
\KwData{A deterministic LTS $\langle Q, q_0, A, \to\rangle$, a state $q_i \in Q$, and a starter $\hat{s} = \{\langle a_1, q_1 \rangle, \hdots , \langle a_n, q_n \rangle \}$ in $q_i$}
\KwResult{A maximal prefix closed diamond $\diamond$ in $q_i$ starting with $\hat{s}$, or \textbf{false} if no such maximal diamond exists.}
$\diamond_H \gets [[a_1], \hdots, [a_n]] $\;
$\textit{qs} \gets \lambda_{\vec{v}}.\bot [\textit{unit}(1) \mapsto q_1, \hdots ,\textit{unit}(n) \mapsto q_n]$\;
$\textit{maxlength} \gets n$\;
$\vec{f} \gets \textit{unit}(1)$\;
\While{$|\vec{f}| < \textit{maxlength}$}{
    $b \gets \vec{f}~\textit{is basic}$\;
    $\textit{edges} \gets [\textbf{false}, \hdots, \textbf{false}]$\;
    $q \gets \textit{qs}(\vec{f})$\;
    \For{$a,q'$ s.t.\ $\textit{qs}(\vec{f}) \xrightarrow{a} q'$}{
        $\textit{found} \gets \bot$\;
        \For{$i \gets 1 ~\KwTo ~n$}{
            $a_i \gets \diamond_H[i, \vec{f}[i]]$\;
            \If{$a_i = a$}{
                $\textit{found} \gets i$\;
                $\textit{edges}[i] \gets \textbf{true}$\;
                \eIf{$\textit{qs}[\vec{f} + \textit{unit}(i)] = \bot$}{
                    $\textit{qs}[\vec{f} + \textit{unit}(i)] \gets q'$\;
                }{
                    \If{$\textit{qs}[\vec{f} + \textit{unit}(i)] \neq q'$}{
                        \textbf{return false}\;
                    }
                }
                \textbf{break}\;
            }
        }
        \If{$\textit{found} = \bot$}{
            \eIf{$b$}{
                $b \gets \textbf{false}$ \;
                $i \gets \textit{base}(\vec{f})$\;
                $\diamond_H[\vec{f}[i], i] \gets a$ \;
                $\textit{maxlength} \gets \textit{maxlength} + 1$ \;
                $\textit{edges}[i] \gets \textbf{true}$\;
                $\textit{qs}[\vec{f} + \textit{unit}(i)] \gets q'$ \;
            }{
                \textbf{return false}\;
            }
        }
    }
    \If{$\textit{edges} \neq [\textbf{true}, \hdots, \textbf{true}]$}{
        \textbf{return false}\;
    }
    $\vec{f}$ shift \;
}
\textbf{return} $\diamond_H$ \;
\end{algorithm}

